Towards the weighted bounded negativity conjecture for blow-ups of algebraic surfaces

In the present paper, we focus on a weighted version of the Bounded Negativity Conjecture which predicts that for every smooth projective surface in characteristic zero the self-intersection numbers of reduced and irreducible curves are bounded from below by a global constant. We gather evidence for this conjecture by showing various bounds on the self-intersection number of curves in an algebraic surface. We focus our attention on blow-ups of algebraic surfaces, which have so far been neglected.

==> extra.tex <==
\section{Comments} 

Please add this comments in the main core of the text. I do not remember your idea about placing them, so I do not want to mess the thing up.\Roberto{We have to think carefully about this: I wouldn't want to write something that will bite us in the ass later. Please let me know if you have some ideas.}

\begin{itemize}
		\item (Roberto) We should come up with a good reason for this paper. Here is one: there seems to be no obvious evidence of why the Weighted BNC should be true. In other words: can we find a big and nef line bundle $L$ such that the Weighted BNC holds with respect to $L$? To me, there is no obvious candidate, unless the surface is of general type, in which case we can take the pull-back of the canonical divisor on the minimal model.
        
        \item (Roberto) On another note, the Weak BNC says that if $\kappa(X) \geq 0$, then 
        \[ C^2 \geq 3e(X) - K_X^2  + 2 - 2g(C). \]
        Now, using adjunction formula, we get 
        \[ C^2 \geq \frac{1}{2} (3e(X) - K_X^2)+\frac{1}{2}(\bar{C}.K_X)= \frac{1}{2}(3e(X) - K_X^2) + \frac{1}{2}(C.\sigma^*K_X),  \]
        but unfortunately $\sigma^*K_X$ is not always big, so we cannot use this even though it provide a perfectly legitimate bound on the self-intersection.
        
        \item (Roberto) In fact, it seems that finding line bundles which help bounding the negativity is not so hard - this is now a big problem for us, because the lack of examples was our motivation for this paper! 
        
        Start with a surface $X$, and write the canonical bundle $K_X$ as the difference of two very ample divisors, $K_X = K_X^+ - K_X^-$. For an irreducible curve $C$, the adjunction formula says
        \[ C^2 =2p_a(C) - 2 - K_X.C \geq -2 - (K_X^+ - K_X^-).C \geq -2 -K_X^+.C \geq -3(K_X^+.C). \]
        So, as you see, it is not hard to come up with a line bundle that does the job, and in fact this shows that $C^2 \geq -3(A.C)$ for all $A \in K_X^+ + \text{Nef}(X)$ (the translate of the nef cone by $K_X^+$).
        
        Now we move to the case of blow-ups of surfaces. Let $\sigma: Y \longra X$ be the blow-up of $X$ at $n$ distinct points $p_1, \dots, p_n$. We seek a connection between the negativity on $X$ and $Y$. For an irreducible curve $C \subset Y$, with image $\bar{C} := \sigma(C)$, one has $C^2 \geq \bar{C}^2 - \sum_{p_i \in \bar{C}} m_{p_i}(\bar{C})^2$. Let us choose a very ample line bundle $H$ on $X$, which clearly gives $m_{p_i} \leq (\bar{C}.H)$ for all $p_i \in \bar{C}$. On the other hand, the adjunction formula on $X$ gives $\bar{C}^2 \geq -2 - (K_X^+.\bar{C})$, and altogether this gives
        \begin{align*}
        	C^2 &\geq -2 - (K_X^+.\bar{C}) - \sum_{p_i \in \bar{C}} (H.\bar{C})^2\\
            &\geq -2 - (K_X^+.\bar{C}) - n(H.\bar{C})^2\\
            &\geq -2 - (K_X^+.\bar{C})^2 - n(H.\bar{C})^2.
        \end{align*}
        Now, if we choose a positive integer $m$ such that $n \leq m^2$, then 
        \begin{align*}
        	C^2 &\geq -2 - (K_X^+.\bar{C})^2 - n(H.\bar{C})^2\\
            &\geq -2 - (K_X^+.\bar{C})^2 - (mH.\bar{C})^2\\
            &\geq -2 - [(K_X^++mH).\bar{C}]^2\\
            &\geq -3(\Delta.{C})^2,
        \end{align*}
        where $\Delta:= \sigma^*(K_X^++mH)$. Again, this shows that we can bound $C^2$ by using any line bundle $A$ on $Y$ with $A \in \Delta + \text{Nef}(Y)$. 
        
        Now let us observe that in the first case the bound is a linear function, but the line bundle is on the surface we start with. In the second case, the bound is a quadratic function on $Y$ but the line bundle comes from a blow-down $X$ of $Y$. In our note, what we are showing is the existence of a linear bound given by a line bundle that comes from a blow-down of the surface we want to study. Is it enough as a reason for having this paper out.

\end{itemize}

\section{Missing cases Hirzebruch}

We are only left with the following cases:
	\begin{itemize}
		\item[(I)] $1 \leq b \leq 2$;
        \item[(II)] $0 \leq a \leq 2 - \frac{1}{2}bm$.
	\end{itemize}
In case (I), $b=1$ implies that an irreducible $C$ of type $(a,1)$ is in fact smooth, since $C.F=1$. Moreover, $C$ must be a section of $\pi: \IF_m \longra \IP^1$. {\color{red} What about the case $b=2$?}

In case (II), we see that necessarily $m \leq 4$. This means that:
\begin{enumerate}
    \item if $m>4$, then case (II) does not occur;
    \item if $m=3,4$, then $b=1$ and $a=0$;
    \item if $m=2$, then either $b=2$ and $a=0$, or $b=1$ and $a \in \lbrace 0,1 \rbrace$;
	\item if $m=0$, then $a \in \lbrace 0,1,2 \rbrace$ (no restriction on $b$).
\end{enumerate}
Notice that we are excluding the case $m=1$, since $\IF_1$ is not minimal. Observe that, by using the genus formula for curves on $\IF_m$, $b=1$ implies that $C$ is smooth and rational. Also, in case (4), $a =1$ implies again that $C \cong \IP^1$ by the same argument.


\section{Infinitely near blow-ups}

We start by looking at an easy example. Let $X = \IP^2$ and let $\sigma:  Y \longra \IP^2$ be a \textit{purely infinitely near blow-up} of $\IP^2$, that is a blow-up of $\IP^2$ concentrated at a single point. This means that $\sigma$ consists in fact of a chain of $n$ blow-ups $\sigma_i : Y_i \longra Y_{i-1}$ such that $Y_0=\IP^2$ and $Y_n = Y$. Let $p_1 \in \IP^2$ be the first point we blow up, $p_2 \in E_1$ be the second, $p_3 \in E_1 \cup E_2$ the third, and so on. Here $E_i$ denotes the exceptional divisor of the $i$\textsuperscript{th} blow-up. 

Let $C$ be an integral curve on $Y$, and let us assume that $C$ is none of the exceptional divisors. Then, the image $\bar{C}:=\sigma(C)$ is an integral curve. Also, let us assume that $p_1 \in {\rm Sing}(\bar{C})$, for otherwise $C^2 \geq \bar{C}^2-n$ since we are blowing up at worst smooth points of $\bar{C}$.

By Theorem \ref{SOZ}, we have that
\begin{align*}
		C^2 &= d^2 - \sum_i m_{p_i}^2 \geq \frac{3}{2}d + \sum_{p \in {\rm Sing}(\bar{C})}\bigg(1 + \frac{1}{2m_{p_{i}}}\bigg)\mu_{p_{i}} - \sum_i m_{p_i}^2\\
        &\geq \frac{3}{2}d + \bigg(1 + \frac{1}{2m_{p_{1}}}\bigg)\mu_{p_{1}} - \sum_i m_{p_i}^2.
\end{align*}

Again, by a result of Milnor \cite{Milnor}, $\mu_{p_1} + r_{p_1} -1 = \sum_j \nu_j(\nu_j-1)$, where $(\nu_j)_j$ is the multiplicity sequence of $p_1$. By plugging in into the inequality above, we get
\begin{align*}
		C^2 &\geq  \frac{3}{2}d + \mu_{p_{1}} - \sum_i m_{p_i}^2 \\
        &\geq \frac{3}{2}d + \sum_j \nu_j(\nu_j-1) + 1 - r_{p_1} - \sum_i m_{p_i}^2\\
        &= \frac{3}{2}d +1 - r_{p_1} - \sum_j\nu_j + \underbrace{\Big[ \sum_j \nu_j^2 - \sum_i m_{p_i}^2 \Big]}_{(\dagger)}.
\end{align*}

Clearly, $r_{p_1} \leq d$, so we need not worry about this term. We do need to bound both $\sum_j \nu_j$ and ($\dagger$). {\color{blue}The idea is that some of the $\nu_j$'s and some of the $m_{p_i}$'s should be related.\newline

\textbf{Assumption:} $\nu_j = m_{p_i}$ if they "correspond to the same point" (or at least $\nu_j \geq m_{p_i}$).\newline

\noindent
If so, we can let $p_1, \dots, p_r$ ($r \leq n$) be the singular points of the intermediate strict transforms of $C$, and $p_{r+1}, \dots, p_n$ be smooth points of an intermediate strict transform of $C$ or points that do not lie on any such curve. Then, we can bound ($\dagger$) as follows:
\[ (\dagger) = \sum {'} (\nu_j^2 - m_{p_i}^2) + \sum {''}\nu_j^2 - \sum {'''} m_{p_i}^2 \geq 0 +0 - n = -n,\]
where $\sum {'}$ is the sum of terms where $j$ and $p_i$ "correspond", $\sum {''}$ is the sum over those $j$'s that are left out in $\sum {'}$, and $\sum {'''}$ is the sum over those $p_i$'s that are left out of $\sum {'}$ (hence these $p_i$'s are not necessary in the resolution process).

It then follows that we obtain the following bound on the self-intersection of $C$:
\[ C^2 \geq \frac{1}{2}d +1 - n - \underbrace{\sum_j \nu_j}_{(\star)}. \]
In order to bound ($\star$), we need to bound the resolution process of $\bar{C}$. I will make the following\newline

\textbf{Claim:} \begin{itemize}
					\item the sequence $(\nu_j)_j$ is non-increasing;
                    \item the length of the sequence $(\nu_j)_j$ is bounded;
				\end{itemize}
                
                
The fact that $(\nu_j)_j$ is non-increasing should be known to experts (reference???), so let us take it for granted. Perhaps this is bounded by $m_{p_1}$ itself, in which case we would have $\sum_j \nu_j \leq \sum_j m_{p_1}$, and we can bound $m_1$ by using the degree $d$. 

Let us now denote by $s$ the length of the multiplicity sequence of a singularity of a curve $D$. Then, we look for a bound of the resolution of singularities (RS) of $D$: 
\begin{align*}
	s &\geq \#\lbrace \text{blow-ups in the very strong RS of $D$} \rbrace\\
    &= \# \lbrace \text{blow-ups in the weak RS of $D$}\rbrace + \#\lbrace \text{blow-ups in the weak RS of $\tilde{D}+ \IE$} \rbrace.
\end{align*}
Now one should be able to find a bound using results in \cite{kollar}...}


